A General Spatio-Temporal Clustering-Based Non-local Formulation for Multiscale Modeling of Compartmentalized Reservoirs

Representing the reservoir as a network of discrete compartments with neighbor and non-neighbor connections is a fast, yet accurate method for analyzing oil and gas reservoirs. Automatic and rapid detection of coarse-scale compartments with distinct static and dynamic properties is an integral part of such high-level reservoir analysis. In this work, we present a hybrid framework specific to reservoir analysis for an automatic detection of clusters in space using spatial and temporal field data, coupled with a physics-based multiscale modeling approach. In this work a novel hybrid approach is presented in which we couple a physics-based non-local modeling framework with data-driven clustering techniques to provide a fast and accurate multiscale modeling of compartmentalized reservoirs. This research also adds to the literature by presenting a comprehensive work on spatio-temporal clustering for reservoir studies applications that well considers the clustering complexities, the intrinsic sparse and noisy nature of the data, and the interpretability of the outcome. Keywords: Artificial Intelligence; Machine Learning; Spatio-Temporal Clustering; Physics-Based Data-Driven Formulation; Multiscale Modeling

==> WRM19_specopyright.tex <==
\scriptsize \noindent Copyright 2019, Society of Petroleum Engineers 
\\
\noindent This paper was prepared for presentation at the SPE Western Regional Meeting held in San Jose, California, U.S.A.,
23-26 April 2019. 
\\
\noindent This paper was selected for presentation by an SPE program
committee following review of information contained in an abstract
submitted by the author(s). Contents of the paper have not been
reviewed by the Society of Petroleum Engineers and are subject to
correction by the author(s). The material does not necessarily
reflect any position of the Society of Petroleum Engineers, its
officers, or members. Electronic reproduction, distribution, or
storage of any part of this paper without the written consent of the
Society of Petroleum Engineers is prohibited. Permission to
reproduce in print is restricted to an abstract of not more than 300
words; illustrations may not be copied. The abstract must contain
conspicuous acknowledgment of SPE copyright.
\vspace*{4pt}
{\color[rgb]{0.28515625,0.57421875,0.859375} \hrule height1pt
  \color[rgb]{0.1328125,0.40625,0.6796875} \hrule height1pt
  \color[rgb]{0.078125,0.2421875,0.40234375} \hrule height1pt}

\normalsize




%\vspace*{10pt}
%\hrule height1pt
%\normalsize





%
%\noindent {\sffamily \scriptsize This paper was prepared for
%  presentation at the 2013 SPE Reservoir Simulation Symposium held in
%  Woodlands, Texas, U.S.A., 18-20 February 2013.}
%\vspace*{5pt}
%
%\noindent {\sffamily \scriptsize This paper was selected for
%  presentation by an SPE Program Committee following review of
%  information contained in an abstract submitted by the
%  author(s). Contents of the paper, as presented, have not been
%  reviewed by the Society of Petroleum Engineers and are subject to
%  correction by the author(s). The material, as presented, does not
%  necessarily reflect any position of the Society of Petroleum
%  Engineers, its officers, or members. Papers presented at SPE
%  meetings are subject to publication review by Editorial Committees
%  of the Society of Petroleum Engineers. Electronic reproduction,
%  distribution, or storage of any part of this paper for commercial
%  purposes without the written consent of the Society of Petroleum
%  Engineers is prohibited. Permission to reproduce in print is
%  restricted to an abstract of not more than 300 words; illustrations
%  may not be copied. The abstract must contain conspicuous
%  acknowledgment of SPE copyright.}
%
%
%\vspace*{10pt}
%{\color[rgb]{0.28515625,0.57421875,0.859375} \hrule height1pt
%  \color[rgb]{0.1328125,0.40625,0.6796875} \hrule height2pt
%  \color[rgb]{0.078125,0.2421875,0.40234375} \hrule height1pt}
%
%\normalsize

==> references_manual <==
\begin{thebibliography}{}

\bibitem[\protect\astroncite{Aach and Church}{2001}]{Aach2001}
Aach, J. and Church, G.~M. (2001).
\newblock {Aligning gene expression time series with time warping algorithms}.
\newblock {\em Bioinformatics}, 17(6):495--508.

\bibitem[\protect\astroncite{Abu-Al-Saud et~al.}{2019}]{moatazaa}
Abu-Al-Saud, M.~O., Esmaeilzadeh, S., and Tchelepi, H.~A. (2019).
\newblock {Insights into the Impact of Water Salinity on Multiphase Flow at the
  Pore-Scale in Carbonate Formations}.
\newblock {\em 21st SPE Middle East Oil and Gas Show and Conference},
  (SPE-194985-MS).

\bibitem[\protect\astroncite{Abu-Al-Saud et~al.}{2016}]{Abu-Al-Saud2016}
Abu-Al-Saud, M.~O., Riaz, A., and Tchelepi, H.~A. (2016).
\newblock {Multiscale level-set method for accurate modeling of immiscible
  two-phase flow with deposited thin films on solid surfaces}.
\newblock {\em Journal of Computational Physics}, 333:297--320.

\bibitem[\protect\astroncite{Aghabozorgi et~al.}{2015}]{Aghabozorgi2015}
Aghabozorgi, S., Seyed~Shirkhorshidi, A., and Ying~Wah, T. (2015).
\newblock {Time-series clustering - A decade review}.
\newblock {\em Information Systems}, 53:16--38.

\bibitem[\protect\astroncite{Ahmad and Dey}{2007}]{Ahmad2007}
Ahmad, A. and Dey, L. (2007).
\newblock {A k-mean clustering algorithm for mixed numeric and categorical
  data}.
\newblock {\em Data and Knowledge Engineering}, 63(2):503--527.

\bibitem[\protect\astroncite{Ahmed}{2006}]{Tarek}
Ahmed, T. (2006).
\newblock {Reservoir Engineering Handbook}.
\newblock {\em Elsevier Inc.}

\bibitem[\protect\astroncite{Alsabti et~al.}{1997}]{Alsabti1997}
Alsabti, K., Ranka, S., and Singh, V. (1997).
\newblock {An efficient k-means clustering algorithm}.
\newblock {\em Electrical Engineering and Computer Science}, 3.

\bibitem[\protect\astroncite{Bar-Joseph et~al.}{2002}]{Bar-Joseph2002}
Bar-Joseph, Z., Gerber, G., Gifford, D.~K., Jaakkola, T.~S., and Simon, I.
  (2002).
\newblock {A new approach to analyzing gene expression time series data}.
\newblock {\em Proceedings of the sixth annual international conference on
  Computational biology - RECOMB '02}, pages 39--48.

\bibitem[\protect\astroncite{Barker and Thibeau}{1997}]{Barker1997}
Barker, J.~W. and Thibeau, S. (1997).
\newblock {A Critical Review of the Use of Pseudorelative Permeabilities for
  Upscaling}.
\newblock {\em SPE Reservoir Engineering}, 12(02):138--143.

\bibitem[\protect\astroncite{Bistrian and Navon}{2017}]{Bistrian2017}
Bistrian, D.~A. and Navon, I.~M. (2017).
\newblock {Randomized dynamic mode decomposition for nonintrusive reduced order
  modelling}.
\newblock {\em International Journal for Numerical Methods in Engineering},
  112(1):3--25.

\bibitem[\protect\astroncite{Bonnet et~al.}{2001}]{Bonnet2001}
Bonnet, E., Bour, O., Odling, N.~E., Davy, P., Main, I., Cowie, P., and
  Berkowitz, B. (2001).
\newblock {Scaling of fractures in geological media}.
\newblock {\em Reviews of Geophysics}, (1999):347--383.

\bibitem[\protect\astroncite{Borah and Bhattacharyya}{2004}]{Borah2004}
Borah, B. and Bhattacharyya, D. (2004).
\newblock {An improved sampling-based DBSCAN for large spatial databases}.
\newblock {\em International Conference on Intelligent Sensing and Information
  Processing, 2004. Proceedings of}, pages 92--96.

\bibitem[\protect\astroncite{Brown et~al.}{2017}]{Brown2017}
Brown, J.~B., Salehi, A., Benhallam, W., and Matringe, S.~F. (2017).
\newblock {Using Data-Driven Technologies to Accelerate the Field Development
  Planning Process for Mature Field Rejuvenation}.
\newblock {\em SPE Western Regional Meeting}, (SPE-185751-MS).

\bibitem[\protect\astroncite{Camacho et~al.}{2017}]{Camacho2017}
Camacho, A., Talavera, A., Emerick, A.~A., Pacheco, M.~A., and Zanni, J.
  (2017).
\newblock {Uncertainty quantification in reservoir simulation models with
  polynomial chaos expansions: Smolyak quadrature and regression method
  approach}.
\newblock {\em Journal of Petroleum Science and Engineering},
  153(March):203--211.

\bibitem[\protect\astroncite{Cardoso and Durlofsky}{2009}]{cardoso2010}
Cardoso, M.~A. and Durlofsky, L.~J. (2009).
\newblock {Use of Reduced-Order Modeling Procedures for Production
  Optimization}.
\newblock {\em SPE Reservoir Simulation Symposium}, (June).

\bibitem[\protect\astroncite{Cardoso et~al.}{2009}]{cardoso2009}
Cardoso, M.~A., {L.J.Durlofsky}, and Sarma, P. (2009).
\newblock {Development and application of reduced-order modeling procedures for
  subsurface flow simulation}.
\newblock {\em International Journal for Numerical Methods in Engineering}.

\bibitem[\protect\astroncite{Chaturvedi et~al.}{2001}]{Chaturvedi2001}
Chaturvedi, A., Foods, K., Green, P.~E., and Carroll, J.~D. (2001).
\newblock {K-modes clustering}.
\newblock {\em Journal of cla}, 18:35--55.

\bibitem[\protect\astroncite{Chatzis}{2008}]{ChatzisSotiriosP.2008}
Chatzis, Sotirios~P., T. A.~V. (2008).
\newblock {Markov Random Field Models for Enhanced Spatially Constrained Image
  Segmentation}.
\newblock {\em October}, 16(5):1351--1361.

\bibitem[\protect\astroncite{Cinar and Riaz}{2014}]{Cinar2014}
Cinar, Y. and Riaz, A. (2014).
\newblock {Carbon dioxide sequestration in saline formations: Part 2-Review of
  multiphase flow modeling}.
\newblock {\em Journal of Petroleum Science and Engineering}, 124:381--398.

\bibitem[\protect\astroncite{Coppi et~al.}{2010}]{Coppi2010}
Coppi, R., D'Urso, P., and Giordani, P. (2010).
\newblock {A fuzzy clustering model for multivariate spatial time series}.
\newblock {\em Journal of Classification}, 27(1):54--88.

\bibitem[\protect\astroncite{Darve}{2000}]{Darve2000}
Darve, E. (2000).
\newblock {Downloaded 04 / 04 / 13 to 171 . 67 . 216 . 21 . Redistribution
  subject to SIAM license or copyright ; see
  http://www.siam.org/journals/ojsa.php}.
\newblock 38(1):98--128.

\bibitem[\protect\astroncite{Durlofsky et~al.}{1996}]{Durlofsky1996}
Durlofsky, L., Behrens, R., Jones, R., and Bernath, A. (1996).
\newblock {Scale Up of Heterogeneous Three Dimensional Reservoir Descriptions}.
\newblock {\em SPE Journal}, 1(03):313--326.

\bibitem[\protect\astroncite{Durlofsky}{1998}]{Durlofsky1998}
Durlofsky, L.~J. (1998).
\newblock {Coarse scale models of two phase flow in heterogeneous reservoirs:
  volume averaged equations and their relationship to existing upscaling
  techniques}.
\newblock {\em Computational Geosciences}, 2(2):73--92.

\bibitem[\protect\astroncite{Esmaeilzadeh and Alam}{2019}]{Esmaeilzadeh2019a}
Esmaeilzadeh, S. and Alam, M.~R. (2019).
\newblock {Shape optimization of wave energy converters for broadband
  directional incident waves}.
\newblock {\em Ocean Engineering}, 174:186--200.

\bibitem[\protect\astroncite{Fetkovich}{1971}]{Fetkovich1971}
Fetkovich, M.~J. (1971).
\newblock {A Simplified Approach to Water Influx Calculations-Finite Aquifer
  Systems}.
\newblock {\em Journal of Petroleum Technology}, 23(07):814--828.

\bibitem[\protect\astroncite{Forsum et~al.}{1978}]{Forsum1978}
Forsum, U., Hjelm, E., Holmberg, K., Nord, C.~E., and Wallin, J. (1978).
\newblock {Genital occurrence of oral microbiota}.
\newblock {\em Acta Dermato-Venereologica}, 58(4):353--356.

\bibitem[\protect\astroncite{Fredrik and Tveito}{1998}]{Fredrik1998}
Fredrik, B. and Tveito, A. (1998).
\newblock {An upscaling method for one-phase flow in heterogeneous reservoirs.
  A weighted output least squares (WOLS) approach}.
\newblock {\em Computational Geosciences}, 2(110673):93--123.

\bibitem[\protect\astroncite{Fujimoto and Scherpen}{2010}]{Fujimoto2010}
Fujimoto, K. and Scherpen, J. M.~A. (2010).
\newblock {Balanced Realization and Model Order Reduction for Nonlinear Systems
  Based on Singular Value Analysis}.
\newblock {\em SIAM Journal on Control and Optimization}, 48(7):4591--4623.

\bibitem[\protect\astroncite{Gautier et~al.}{1999}]{Gautier1999}
Gautier, Y., Blunt, M., and Christie, M. (1999).
\newblock {Nested Gridding and Streamline-Based Simulation for Fast Reservoir
  Performance Prediction}.
\newblock {\em Reservoir Simulation Symposium}, 3(1):1--10.

\bibitem[\protect\astroncite{Gavrila and Davis}{1995}]{Gavrila1995}
Gavrila, D.~M. and Davis, L.~S. (1995).
\newblock {Towards 3-D model-based tracking and recognition of human movement:
  a multi-view approach}.
\newblock {\em In International Workshop on Automatic Face- and
  Gesture-Recognition. IEEE Computer Society}, 3(6):272--277.

\bibitem[\protect\astroncite{Gharib~Shirangi}{2014}]{GharibShirangi2014}
Gharib~Shirangi, M. (2014).
\newblock {History matching production data and uncertainty assessment with an
  efficient TSVD parameterization algorithm}.
\newblock {\em Journal of Petroleum Science and Engineering}, 113:54--71.

\bibitem[\protect\astroncite{Ghasemi et~al.}{2014}]{Ghasemi2014}
Ghasemi, M., Ibrahim, A., and Gildin, E. (2014).
\newblock {Reduced Order Modeling In Reservoir Simulation Using the Bilinear
  Approximation Techniques}.
\newblock {\em SPE Latin America and Caribbean Petroleum Engineering
  Conference}.

\bibitem[\protect\astroncite{Ghasemi et~al.}{2012}]{Ghasemi2012}
Ghasemi, M., Zhao, S., Insperger, T., and Kalm{\'{a}}r-Nagy, T. (2012).
\newblock {Act-and-wait control of discrete systems with random delays}.
\newblock {\em Proceedings of the American Control Conference}, pages
  5440--5443.

\bibitem[\protect\astroncite{Gildin and Lopez}{2011}]{Gildin2011}
Gildin, E. and Lopez, T. (2011).
\newblock {Closed-Loop Reservoir Management: Do we need complex models?}
\newblock {\em SPE Digital Energy Conference and Exhibition}, pages 19--21.

\bibitem[\protect\astroncite{Hajibeygi and Jenny}{2009}]{Hajibeygi2009}
Hajibeygi, H. and Jenny, P. (2009).
\newblock {Multiscale finite-volume method for parabolic problems arising from
  compressible multiphase flow in porous media}.
\newblock {\em Journal of Computational Physics}, 228(14):5129--5147.

\bibitem[\protect\astroncite{Hajibeygi and Jenny}{2011}]{Hajibeygi2011}
Hajibeygi, H. and Jenny, P. (2011).
\newblock {Adaptive iterative multiscale finite volume method}.
\newblock {\em Journal of Computational Physics}, 230(3):628--643.

\bibitem[\protect\astroncite{Hajibeygi et~al.}{2012}]{Hajibeygi2012}
Hajibeygi, H., Lee, S.~H., and Lunati, I. (2012).
\newblock {Accurate and Efficient Simulation of Multiphase Flow in a
  Heterogeneous Reservoir With Error Estimate and Control in the Multiscale
  Finite-Volume Framework}.
\newblock {\em Spe Journal}, 17(4):1071--1083.

\bibitem[\protect\astroncite{Hartigan and Wong}{1979}]{Hartigan1979}
Hartigan, J.~A. and Wong, M.~A. (1979).
\newblock {Algorithm AS 136: A K-Means Clustering Algorithm}.
\newblock 28(1):100--108.

\bibitem[\protect\astroncite{Heijn et~al.}{2004}]{Heijn2004}
Heijn, T., Markovinovi{\'{c}}, R., and Jansen, J.-D. (2004).
\newblock {Generation of Low-Order Reservoir Models Using System-Theoretical
  Concepts}.
\newblock {\em SPE Journal}, 9(2):3--5.

\bibitem[\protect\astroncite{Hiroaki and Seibi}{1978}]{Hiroaki1978}
Hiroaki, S. and Seibi, C. (1978).
\newblock {Dynamic programming algorithm optimization for spoken word
  recognition}.
\newblock {\em Ieee Transactions on Acoustics, Speech, and Signal Processing,},
  ASSP-26(February):43--49.

\bibitem[\protect\astroncite{Holden and Nielsen}{2000}]{Holden2000}
Holden, L. and Nielsen, B.~F. (2000).
\newblock {Global upscaling of permeability in heterogeneous reservoirs; the
  Output Least Squares (OLS) method}.
\newblock {\em Transport in Porous Media}, 40(2):115--143.

\bibitem[\protect\astroncite{Huang}{1997}]{LiJie}
Huang, Z. (1997).
\newblock {Clustering Large Data Sets With Mixed Numeric And Categorical
  Values}.
\newblock {\em In The First Pacific-Asia Conference on Knowledge Discovery and
  Data Mining}.

\bibitem[\protect\astroncite{Huang}{1998}]{Zhexue1998}
Huang, Z. (1998).
\newblock {Extensions to the k-Means Algorithm for Clustering Large Data Sets
  with Categorical Values}.
\newblock {\em Data Mining and Knowledge Discovery}, 2:283--304.

\bibitem[\protect\astroncite{Huang and K.~Ng}{1999}]{Huang1999}
Huang, Z. and K.~Ng, M. (1999).
\newblock {A Fuzzy k-Modes Algorithm for Clustering Categorical Data}.
\newblock {\em IEEE Transactions on Fuzzy Systems}, 7(4):661--666.

\bibitem[\protect\astroncite{Huang and Ng}{2003}]{Huang2003}
Huang, Z. and Ng, M.~K. (2003).
\newblock {A Note on K-modes Clustering}.
\newblock {\em Journal of Classification}, 20(2):257--261.

\bibitem[\protect\astroncite{Jain}{2010}]{Jain2010}
Jain, A.~K. (2010).
\newblock {Data clustering: 50 years beyond K-means}.
\newblock {\em Pattern Recognition Letters}, 31(8):651--666.

\bibitem[\protect\astroncite{Ji et~al.}{2012}]{Ji2012}
Ji, J., Pang, W., Zhou, C., Han, X., and Wang, Z. (2012).
\newblock {A fuzzy k-prototype clustering algorithm for mixed numeric and
  categorical data}.
\newblock {\em Knowledge-Based Systems}, 30:129--135.

\bibitem[\protect\astroncite{Kruskall and Liberman}{1983}]{Kruskall1983}
Kruskall, J.~B. and Liberman, M. (1983).
\newblock {The symmetric time warping algorithm: From continuous to discrete}.
\newblock {\em Time Warps, String Edits and Macromolecules},
  (July):125{\~{}}161.

\bibitem[\protect\astroncite{Lee et~al.}{2014}]{Lee2014a}
Lee, K., Jung, S., Shin, H., and Choe, J. (2014).
\newblock {Uncertainty Quantification of Channelized Reservoir Using Ensemble
  Smoother with Selective Measurement Data}.
\newblock {\em Energy Exploration {\&} Exploitation}, 32(5):805--816.

\bibitem[\protect\astroncite{Lee et~al.}{2008}]{Lee2008}
Lee, S.~H., Wolfsteiner, C., and Tchelepi, H.~A. (2008).
\newblock {Multiscale finite-volume formulation for multiphase flow in porous
  media: Black oil formulation of compressible, three-phase flow with gravity}.
\newblock {\em Computational Geosciences}, 12(3):351--366.

\bibitem[\protect\astroncite{Legendre}{1987}]{Legendre1987}
Legendre, P. (1987).
\newblock {\em {Constrained clustering}}, volume G14.

\bibitem[\protect\astroncite{Lin and Chih-Jen}{2012}]{Lin2012}
Lin, C.-W.~H. and Chih-Jen (2012).
\newblock {Machines, A Comparison of Methods for Multi-class Support Vector}.
\newblock 13(2):415--425.

\bibitem[\protect\astroncite{Ma et~al.}{2017}]{Bi2017}
Ma, X., Hetz, G., Wang, X., Bi, L., Stern, D., and Hoda, N. (2017).
\newblock {A Robust Iterative Ensemble Smoother Method for Efficient History
  Matching and Uncertainty Quantification}.

\bibitem[\protect\astroncite{Markovinvi{\'{c}} et~al.}{2002}]{Markovinvic2002}
Markovinvi{\'{c}}, R., Geurtsen, E.~L., and Jansen, J.~D. (2002).
\newblock {Subspace identification of low-order reservoir models}.
\newblock {\em Developments in Water Science}, 47(C):281--288.

\bibitem[\protect\astroncite{Matringe et~al.}{2018}]{patent:20150346010}
Matringe, S.~F., Castineira, D., and Salehi, A. (2018).
\newblock {MULTI-TANK MATERIAL BALANCE MODEL}.

\bibitem[\protect\astroncite{Mingjin}{2005}]{Yan2005}
Mingjin, Y. (2005).
\newblock {Methods of Determining the Number of Clusters in a Data Set and a
  New Clustering Criterion}.

\bibitem[\protect\astroncite{Muskat}{1945}]{Muskat1945}
Muskat, M. (1945).
\newblock {The production histories of oil producing gas-drive reservoirs}.
\newblock {\em Journal of Applied Physics}, 16(3):147--159.

\bibitem[\protect\astroncite{Olalotiti et~al.}{2019}]{Olalotiti2019}
Olalotiti, F., Salehi, A., Hetz, G., and Castineira, D. (2019).
\newblock {Application of Flow Diagnostics to Rapid Production Data Integration
  in Complex Geologic Grids and Dual Permeability Models}.
\newblock {\em SPE Western Regional Meeting}, (SPE-195253-MS).

\bibitem[\protect\astroncite{Patil et~al.}{2006}]{Patil2006}
Patil, G.~P., Modarres, R., Myers, W.~L., and Patankar, P. (2006).
\newblock {Spatially constrained clustering and upper level set scan hotspot
  detection in surveillance geoinformatics}.
\newblock {\em Environmental and Ecological Statistics}, 13(4):365--377.

\bibitem[\protect\astroncite{Rabahy and Ignarra}{2002}]{Rabahy2002}
Rabahy, W.~A. and Ignarra, L.~R. (2002).
\newblock {Estudo sobre o Turismo Praticado em Ambientes Naturais Conservados}.
\newblock 2(2):1--170.

\bibitem[\protect\astroncite{Rani and Sikka}{2012}]{Rani2012}
Rani, S. and Sikka, G. (2012).
\newblock {Recent Techniques of Clustering of Time Series Data: A Survey}.
\newblock {\em International Journal of Computer Applications}, 52(15):1--9.

\bibitem[\protect\astroncite{Rath and Manmatha}{}]{Rath}
Rath, T. and Manmatha, R.
\newblock {Word image matching using dynamic time warping}.
\newblock {\em 2003 IEEE Computer Society Conference on Computer Vision and
  Pattern Recognition, 2003. Proceedings.}, 2:II--521--II--527.

\bibitem[\protect\astroncite{Rousseeuw}{1987}]{Pearce1977}
Rousseeuw, P.~J. (1987).
\newblock {Silhouettes: A graphical aid to the interpretation and validation of
  cluster analysis}.
\newblock {\em Journal of Computational and Applied Mathematics}, 20(4):53--65.

\bibitem[\protect\astroncite{Sakoe and Chiba}{1971}]{SakoeChiba71}
Sakoe, H. and Chiba, S. (1971).
\newblock {A Dynamic Programming Approach to Continuous Speech Recognition}.
\newblock In {\em Proceedings of the Seventh International Congress on
  Acoustics, Budapest}, volume~3, pages 65--69, Budapest.

\bibitem[\protect\astroncite{Salehi}{2016}]{Salehi2016}
Salehi, A. (2016).
\newblock {\em {Upscaling of Compositional Flow Simulation Based on a
  Non-Equilibrium Formulation}}.
\newblock PhD thesis, Stanford University.

\bibitem[\protect\astroncite{Salehi et~al.}{2019a}]{Salehi2019a}
Salehi, A., Hetz, G., Olalotiti, F., Sorek, N., Darabi, H., and Castineira, D.
  (2019a).
\newblock {A Comprehensive Adaptive Forecasting Framework for Optimum Field
  Development Planning}.
\newblock {\em SPE Reservoir Simulation Conference}, (SPE-193914-MS).

\bibitem[\protect\astroncite{Salehi et~al.}{2013}]{salehi2013}
Salehi, A., Voskov, D., and Tchelepi, H. (2013).
\newblock {Thermodynamically Consistent Transport Coefficients for Upscaling of
  Compositional Processes}.
\newblock {\em Society of Petroleum Engineers Reservoir Simulation Conference},
  (SPE-163576-MS).

\bibitem[\protect\astroncite{Salehi et~al.}{2019b}]{Salehi2019}
Salehi, A., Voskov, D., and Tchelepi, H. (2019b).
\newblock {K-Values-Based Upscaling of Compositional Simulation}.
\newblock {\em SPE Journal}, (SPE-182725-PA).

\bibitem[\protect\astroncite{Salehi et~al.}{2017}]{Salehi2017}
Salehi, A., Voskov, D.~V., and Tchelepi, H.~A. (2017).
\newblock {K-Values Based Non-Equilibrium Formulation for Upscaling of
  Compositional Simulation}.
\newblock {\em SPE Reservoir Simulation Conference}, (SPE-182725-MS).

\bibitem[\protect\astroncite{Scholkopf and
  Smola}{2001}]{Scholkopf:2001:LKS:559923}
Scholkopf, B. and Smola, A.~J. (2001).
\newblock {\em {Learning with Kernels: Support Vector Machines, Regularization,
  Optimization, and Beyond}}.
\newblock MIT Press, Cambridge, MA, USA.

\bibitem[\protect\astroncite{Scholkopf et~al.}{1998}]{Scholkopf1998}
Scholkopf, M.~H., Dumais, S., B., E.~O., and Platt, J. (1998).
\newblock {Support vector machines}.
\newblock {\em International Journal of Clinical and Experimental Medicine},
  13(4):18--28.

\bibitem[\protect\astroncite{Shirangi and Durlofsky}{2016}]{Shirangi2016}
Shirangi, M.~G. and Durlofsky, L.~J. (2016).
\newblock {A general method to select representative models for decision making
  and optimization under uncertainty}.
\newblock {\em Computers and Geosciences}, 96:109--123.

\bibitem[\protect\astroncite{Steinley}{2006}]{Steinley2006}
Steinley, D. (2006).
\newblock {K-means clustering: A half-century synthesis}.
\newblock {\em British Journal of Mathematical and Statistical Psychology},
  59(1):1--34.

\bibitem[\protect\astroncite{Sugar and James}{2003}]{Sugar2003}
Sugar, C.~A. and James, G.~M. (2003).
\newblock {Finding the Number of Clusters in a Dataset: An
  Information-Theoretic Approach}.
\newblock {\em Journal of the American Statistical Association},
  98(463):750--763.

\bibitem[\protect\astroncite{Suykens and Vandewalle}{1999}]{Suykens1999}
Suykens, J.~A. and Vandewalle, J. (1999).
\newblock {Least squares support vector machine classifiers}.
\newblock {\em Neural Processing Letters}, 9(3):293--300.

\bibitem[\protect\astroncite{Tahmasebi et~al.}{2018}]{Tahmasebi2018}
Tahmasebi, P., Sahimi, M., and Shirangi, M.~G. (2018).
\newblock {Rapid Learning-Based and Geologically Consistent History Matching}.
\newblock {\em Transport in Porous Media}, 122(2):279--304.

\bibitem[\protect\astroncite{Tarner}{1944}]{Tarner}
Tarner, J. (1944).
\newblock {How Different Size Gas Caps and Pressure Maintenance Programs Affect
  Amount of Recoverable Oil}.
\newblock {\em Oil Weekly}, 144.

\bibitem[\protect\astroncite{Tchelepi et~al.}{2007}]{Tchelepi2007}
Tchelepi, H.~A., Jenny, P., Lee, S.~H., and Wolfsteiner, C. (2007).
\newblock {Adaptive Multiscale Finite-Volume Framework for Reservoir
  Simulation}.
\newblock {\em SPE Journal}, 12(02):188--195.

\bibitem[\protect\astroncite{Tracy}{1995}]{Tracy1995}
Tracy, G. (1995).
\newblock {Simplified Form of the MBE}.
\newblock {\em Trans. AIME}, 204:243--246.

\bibitem[\protect\astroncite{Udy et~al.}{2017}]{Udy2017}
Udy, J., Blackburn, L., Hedengren, J.~D., and Darby, M. (2017).
\newblock {Reduced Order Modeling for Reservoir Injection Optimization and
  Forecasting}.
\newblock {\em Foundations of Computer Aided Process Operations / Chemical
  Process Control}.

\bibitem[\protect\astroncite{Vermeulen et~al.}{2004}]{Vermeulen2004}
Vermeulen, P.~T., Heemink, A.~W., and Te~Stroet, C.~B. (2004).
\newblock {Reduced models for linear groundwater flow models using empirical
  orthogonal functions}.
\newblock {\em Advances in Water Resources}, 27(1):57--69.

\bibitem[\protect\astroncite{Wang}{2005}]{9783540243885}
Wang, L. (2005).
\newblock {\em {Support Vector Machines: Theory and Applications}}.
\newblock Springer.

\bibitem[\protect\astroncite{Wen and
  G{\'{o}}mez-Hern{\'{a}}ndez}{1998}]{Wen1998}
Wen, X.~H. and G{\'{o}}mez-Hern{\'{a}}ndez, J.~J. (1998).
\newblock {Upscaling Hydraulic Conductivities in Cross-Bedded Formations}.
\newblock {\em Mathematical Geology}, 30(2):181--211.

\bibitem[\protect\astroncite{Yang et~al.}{2007}]{Yang2007}
Yang, C., Nghiem, L.~X., Card, C., and Bremeier, M. (2007).
\newblock {Reservoir Model Uncertainty Quantification Through Computer-Assisted
  History Matching}.
\newblock {\em SPE Annual Technical Conference and Exhibition}.

\bibitem[\protect\astroncite{Yeh et~al.}{2014}]{Yeh2014}
Yeh, T.-H., Jimenez, E., Van~Essen, G., Chen, C., Jin, L., Girardi, A.,
  Gelderblom, P., Horesh, L., and Conn, A.~R. (2014).
\newblock {Reservoir Uncertainty Quantification Using Probabilistic History
  Matching Workflow}.
\newblock {\em SPE Annual Technical Conference and Exhibition}.

\bibitem[\protect\astroncite{Yeten et~al.}{2003}]{Durlofsky2003}
Yeten, B., Durlofsky, L.~J., and Aziz, K. (2003).
\newblock {Optimization of nonconventional well type, location, and
  trajectory}.
\newblock {\em SPE Journal}, 8(3):200.

\bibitem[\protect\astroncite{Yu et~al.}{2014}]{Yu2014}
Yu, H., Liu, Z., and Wang, G. (2014).
\newblock {An automatic method to determine the number of clusters using
  decision-theoretic rough set}.
\newblock {\em International Journal of Approximate Reasoning}, 55(1 PART
  2):101--115.

\end{thebibliography}

